StreamFP: Learnable Fingerprint-guided Data Selection for Efficient Stream Learning

Stream Learning (SL) requires models that can quickly adapt to continuously evolving data, posing significant challenges in both computational efficiency and learning accuracy. Effective data selection is critical in SL to ensure a balance between information retention and training efficiency. Traditional rule-based data selection methods struggle to accommodate the dynamic nature of streaming data, highlighting the necessity for innovative solutions that effectively address these challenges. Recent approaches to handling changing data distributions face challenges that limit their effectiveness in fast-paced environments. In response, we propose StreamFP, a novel approach that uniquely employs dynamic, learnable parameters called fingerprints to enhance data selection efficiency and adaptability in stream learning. StreamFP optimizes coreset selection through its unique fingerprint-guided mechanism for efficient training while ensuring robust buffer updates that adaptively respond to data dynamics, setting it apart from existing methods in stream learning. Experimental results demonstrate that StreamFP outperforms state-of-the-art methods by achieving accuracy improvements of 15.99%, 29.65%, and 51.24% compared to baseline models across varying data arrival rates, alongside a training throughput increase of 4.6x.

==> Body/5_4_Impl.tex <==
\section{Implementation and Limitations}
This section provides a comprehensive overview of the \system algorithmic details, and its inherent limitations.

% \cc{Any "code level" implementation details that we may emphsize here?}

\subsection{Algorithm Details}
The \system algorithm is summarized in Alg.~\ref{alg:system}. Upon receiving an incoming batch $B^t$, \system begins by selecting a coreset $C^t$ to guide the model update (lines 1-2). The model is then iteratively trained using mini-batches drawn from both $C^t$ and the previous buffer $M^{t-1}$, with fingerprints being refined through the fingerprint-based continual learning mechanism (lines 3-16). After completing the model's training on $B^t$, the buffer is updated from $M^{t-1}$ to $M^t$ using the information in $B^t$ (lines 17-18).

\begin{algorithm} [t]
\caption{\system Overview}
\label{alg:system}
\begin{algorithmic}[1]
\fontsize{8.75}{11}\selectfont
\Statex \textbf{Input:} incoming data batch $B^t$, previous buffer $M^{t-1}$, previous fingerprint parameters $P$, frozen model parameters $\theta$, learnable fingerprint feature refiner $\theta_f$
\Statex \textbf{Output:} updated fingerprint feature refiner $\theta_f$, updated fingerprint parameters $P$ and buffer $M^t$
\State \codecomment{// stage 1: Coreset Selection as detailed in Sec.\ref{sec:pcs}}
\State $C^t \gets \text{CoresetSelection}(B^t)$

\State \codecomment{// stage 2: Model Update}
\State $B_C \gets \text{LoadMiniBatch}(C^t)$ \codecomment{// load by random retrieval}
\State $B_M \gets \text{LoadMiniBatch}(M^{t-1})$
\State $B_{\text{train}} = B_C \cup B_M$
\State \codecomment{// fingerprint attunement as detailed in Sec.\ref{sec:pa}}
\State $P=\theta_f(P; B)$ 
\State \codecomment{// fingerprint-based continual learning}
\State $\mathcal{L} \gets \text{ModelForward}(B, P)$
\State Compute loss $\mathcal{L}$ and perform gradient descent
\State update fingerprint parameters $P$
\State update fingerprint feature refiner $\theta_f$
\State $C^t \gets C^t\setminus B_C$

\State \codecomment{// stage 3: Buffer Update as detailed in Sec.\ref{sec:pbm}}
\State $M^t \gets \text{BufferUpdate}(B^t, M^{t-1})$
\end{algorithmic}
\end{algorithm}

\subsection{Limitations} 
\label{sec:limitations}
One limitation of \system is its reliance on pre-trained components, such as vision transformers, which may not always be available or suitable for all scenarios. Although this reliance is common in current SL methods, there are situations where appropriate pre-trained models are lacking. However, as a framework designed for efficiency, \system has the potential to adapt to various SL methods.
%
For example, integrating alternative architectures or reducing dependency on pre-trained models could make \system more versatile.
%
Another limitation is the computational overhead introduced by the dynamic nature of the fingerprints, which can be particularly challenging in high-velocity or large-volume data streams. Despite the ``Fingerprint Attunement'' mechanism's design to minimize these demands, further optimization is needed to enhance scalability and performance in industrial-scale applications.
%
Moreover, the current evaluations are limited to specific SL tasks, predominantly in the vision domain. While this is a common practice, evaluating \system, as well as other SL methods, on datasets from other domains, such as text and audio, would provide a more comprehensive and reliable assessment.
%
Future work will explore the integration of advanced optimization techniques and the application of \system in non-visual domains, such as text and audio, to evaluate its adaptability and effectiveness across various data types.

==> Body/9_Availability.tex <==
\section*{Availability}
All source code, data, and scripts to reproduce our work is at \url{https://anonymous.4open.science/r/StreamLearning-1F77/}.
